CAP-VMs: Capability-Based Isolation and Sharing for Microservices

Cloud stacks must isolate application components, while permitting efficient data sharing between components deployed on the same physical host. Traditionally, the MMU enforces isolation and permits sharing at page granularity. MMU approaches, however, lead to cloud stacks with large TCBs in kernel space, and page granularity requires inefficient OS interfaces for data sharing. Forthcoming CPUs with hardware support for memory capabilities offer new opportunities to implement isolation and sharing at a finer granularity. We describe cVMs, a new VM-like abstraction that uses memory capabilities to isolate application components while supporting efficient data sharing, all without mandating application code to be capability-aware. cVMs share a single virtual address space safely, each having only capabilities to access its own memory. A cVM may include a library OS, thus minimizing its dependency on the cloud environment. cVMs efficiently exchange data through two capability-based primitives assisted by a small trusted monitor: (i) an asynchronous read-write interface to buffers shared between cVMs; and (ii) a call interface to transfer control between cVMs. Using these two primitives, we build more expressive mechanisms for efficient cross-cVM communication. Our prototype implementation using CHERI RISC-V capabilities shows that cVMs isolate services (Redis and Python) with low overhead while improving data sharing.

==> img/tab.tex <==
% \begin{comment}
% \begin{table}[tb]
%   \centering\footnotesize
%   \caption{\coffer application throughput}\label{tab:total}
% \begin{tabular}{lcc@{}cc@{}c}
% \toprule
%            & \multicolumn{2}{c}{Redis (r/s)}                                                                                      & \multicolumn{2}{c}{AES (MB/s)} &                                                                             \\ \cline{2-6} 
%            & \begin{tabular}[c]{@{}c@{}}SET\end{tabular} & \begin{tabular}[c]{@{}c@{}}GET\end{tabular} & \begin{tabular}[c]{@{}c@{}} enc\end{tabular} & \begin{tabular}[c]{@{}c@{}}dec\end{tabular} & \begin{tabular}[c]{@{}c@{}}\end{tabular} \\ \hline
% Baseline & 4.6\unit{reqs/s} & 5.2\unit{reqs/s} & 0.79 & 0.96 &     \\
%  \magic{} & 5.8\unit{reqs/s} & 7.1\unit{reqs/s} & 0.74 & 0.85 &  \\
%   \bottomrule
% \end{tabular}
% \end{table}
% \end{comment}

\begin{table}[tb]
  \centering\footnotesize
  \caption{Redis and Python throughput \textnormal{(FPGA CHERI)} \noteprp{only
      leave the Python results here?}}\label{tab:total}
  \begin{tabular}{lcc|cc}
    \toprule
    & \multicolumn{2}{c}{\textbf{Redis FPGA}} & \multicolumn{2}{c}{\textbf{Python}} \\ 
    & set & get & enc & dec \\ \midrule
    \textbf{baseline} & 32.3\unit{req/s} & 36.9\unit{req/s} & 0.79\unit{MB/s} & 0.96\unit{MB/s} \\
    \textbf{\magic{}} & 50\unit{req/s} & 57\unit{req/s} & 0.74\unit{MB/s} & 0.85\unit{MB/s} \\
    \bottomrule
  \end{tabular}
\end{table}


==> src/80-unused.tex <==
\newpage
\section{Unused}
\subsubsection{FILES vs CAPFILES: TERM FREQUENCY}

\notevs{These two benchmarks are neither micro nor macro. }

\notevs{By nature, this benchmark is not a microbenchmark. But it is too simple for macro benchmark. can we call it midi benchmark?}
\notevs{Conceptually, the second macro benchmark (python library) shows the same, or kind of the same. So I am not sure that to do with this benchmark and where to put it}

\acsp{capfile} can be used not only for communication between two \glspl{box}, but as a replacement for ordinary files.
We compare the performance of \acsp{capfile} and files located in RAM drive.
For that, we created several files of various sizes, from XX to YY with step ZZ, and implemented a simple data-mining program.
It computes Term Frequency for a given file, which is one of the fundamental metrics in the text analysis.
This metric does not require significant CPU computations, thus we can run it on an FPGA board.

\begin{figure}[h]
  \centering
	\includegraphics[width=1.0\linewidth]{img/tf.png}
  \caption{TF}
  \label{fig:tf}
\end{figure}

\input{img/speedtest1.tex}


Fig.~\ref{fig:tf} depicts the results of the benchmark.
Good start, then converged due to the increasing computational overhead.

\subsubsection{CINVOKE performance: the cost of isolation for LKL}


\todo{There are two benchmarks we can use. Firstly, there is speedtest1 (fig. ~\ref{fig:speedtest}). We used it already in the previous paper, maybe it is not super smart to use it again. However, this benchmark reviles inefficiency in the syscalls interface. If you remember, the isolation of RAMFS lead to significant performance drop. In our case, when any syscall is accompanied by CINVOKE, we don't see any impact. so I vote for speedtest1. I can measure time of each separate query, remove noise, and then diagrams will be identical.}

\todo{The option number two is TPC-C. I generated a database and a query log for 1 warehouse (db is near 98MiB). I generated this log from apavlo's tpcc-benchmark. So, I can reliably repeat this log, measure performance of each query, remove noise, and we will get clean results (if each query fits into a scheduling time-slice, which might be not the case. I don't like this option because TPC-C is not micro benchmark, but two papers in the row with speedtest1?... dunno}. 

\todo{Great diagram that shows nothing. I do not want to use again speedtest, but it might be interesting because we know the overhead of CubicleOS}

\todo{As one can see, there is no visible difference with or without separation between LKL and musl. it is either because it is negligible, or noise overcomes everything.}

\begin{figure}[h]
  \centering
  \begin{tikzpicture}
  \begin{axis}[
		legend style={at={(0.25,0.55)},anchor=south, font=\scriptsize},
		width  = 1.0\linewidth,
		height = 4.5cm,
    enlarge x limits=0.2,
    ybar, ymin=0,ymax=1100,
    bar width=8mm,
%    symbolic x coords={a,b, c, d},
    xticklabels={CAPFILE (m),CAPFILE, CAPDMA, TCP/IP},
    xtick=data,
    ylabel={time (microseconds)},
           ylabel near ticks,
    nodes near coords, 
%    nodes near coords align={anchor=north},%Move values in bar
    every node near coord/.style={yshift=0.2cm
    },
  ]

 \addplot [fill=ACMBlue, error bars/.cd, y dir=both, y explicit relative] coordinates {
	(1,81.636) 
	(2,84.101)
	(3,259.632)
	(4,852.493)
};
%	(4,852.493) +- (0,0.08)
  \end{axis}
  \end{tikzpicture}
  \caption{Ping-Pong time over different communication mechanisms}
  \label{fig:eva:capvstcp-unused}
  \notevs{Probably I will remake this benchmark}
\end{figure}

